Supervised Contrastive Learning

Contrastive learning applied to self-supervised representation learning has seen a resurgence in recent years, leading to state of the art performance in the unsupervised training of deep image models. Modern batch contrastive approaches subsume or significantly outperform traditional contrastive losses such as triplet, max-margin and the N-pairs loss. In this work, we extend the self-supervised batch contrastive approach to the fully-supervised setting, allowing us to effectively leverage label information. Clusters of points belonging to the same class are pulled together in embedding space, while simultaneously pushing apart clusters of samples from different classes. We analyze two possible versions of the supervised contrastive (SupCon) loss, identifying the best-performing formulation of the loss. On ResNet-200, we achieve top-1 accuracy of 81.4% on the ImageNet dataset, which is 0.8% above the best number reported for this architecture. We show consistent outperformance over cross-entropy on other datasets and two ResNet variants. The loss shows benefits for robustness to natural corruptions and is more stable to hyperparameter settings such as optimizers and data augmentations. Our loss function is simple to implement, and reference TensorFlow code is released at https://t.ly/supcon.

==> discussion.tex <==
\section{Discussion}
We have presented a novel loss, inspired by contrastive learning, that outperforms cross entropy on classification accuracy and robustness benchmarks. Furthermore, our experiments show that this loss is less sensitive to hyperparameter changes, which is a useful practical consideration. The loss function provides a natural connection between fully unsupervised training on the one end, and fully supervised training on the other. This opens the possibility of applications in semi-supervised learning which can leverage the benefits of a single loss that can smoothly shift behavior based on the availability of labeled data.

==> gradient.tex <==
\section{Derivation of Supervised Contrastive Learning Gradient}
\label{sec:gradient_derivation}
In Sec 2 in the main paper, we presented motivation based on the functional form of the gradient of the supervised contrastive loss, $\mathcal{L}_i^{sup}(\boldsymbol{z}_i)$ (Eq. 4 in the paper), that the supervised contrastive loss intrinsically causes learning to focus on \emph{hard} positives and negatives, where the encoder can greatly benefit, instead of easy ones, where the encoder can only minimally benefit. In this section, we derive the mathematical expression for the gradient:
\begin{equation}
  \frac{\partial\mathcal{L}_i^{sup}(\boldsymbol{z}_i)}{\partial\boldsymbol{w}_i}=\frac{\partial\boldsymbol{z}_i}{\partial\boldsymbol{w}_i}\cdot\frac{\partial\mathcal{L}_i^{sup}(\boldsymbol{z}_i)}{\partial\boldsymbol{z}_i} \label{gradient_chain_ruile}
\end{equation}
where $\boldsymbol{w}_i$ is the projection network output \emph{prior} to normalization, i.e., $\boldsymbol{z}_i=\boldsymbol{w}_i/\Vert\boldsymbol{w}_i\Vert$. As we will show, normalizing the representations provides structure to the gradient that causes learning to focus on hard positives and negatives instead of easy ones.

The supervised contrastive loss can be rewritten as:
\begin{eqnarray}
  \mathcal{L}_i^{sup}(\boldsymbol{z}_i) & = & \frac{-1}{2N_{\boldsymbol{\tilde{y}}_i}-1}\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot\log{\frac{\exp{\left(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j/\tau\right)}}{\sum_{k=1}^{2N}\mathbbm{1}_{i\neq k}\cdot\exp{\left(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_k/\tau\right)}}}\nonumber\\
  & = & \frac{-1}{2N_{\boldsymbol{\tilde{y}}_i}-1}
  \sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot\left(\frac{\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j}{\tau}-\log{\sum_{k=1}^{2N}\mathbbm{1}_{i\neq k}\cdot\exp{\frac{\boldsymbol{z}_i\bigcdot\boldsymbol{z}_k}{\tau}}}\right)\nonumber
\end{eqnarray}
Thus:
\begin{eqnarray}
  \frac{\partial\mathcal{L}_i^{sup}(\boldsymbol{z}_i)}{\partial\boldsymbol{z}_i} & = & \frac{-1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  \left(
    \boldsymbol{z}_j
    -\sum_{k=1}^{2N}\frac{\mathbbm{1}_{i\neq k}\cdot\boldsymbol{z}_k\cdot\exp{(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_k/\tau)}}{\sum_{m=1}^{2N}\mathbbm{1}_{i\neq m}\cdot\exp{(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_m/\tau)}}
  \right) \nonumber \\
  & = & \frac{-1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  \left(
    \boldsymbol{z}_j-\sum_{k=1}^{2N}\mathbbm{1}_{i\neq k}\cdot\boldsymbol{z}_k\cdot P_{ik}
  \right) \nonumber \\
  & = & \frac{-1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  \left(
    (1-P_{ij})\cdot\boldsymbol{z}_j-\sum_{k=1}^{2N}\mathbbm{1}_{k\notin\{i,j\}}\cdot\boldsymbol{z}_k\cdot P_{ik}
  \right) \label{eq:dloss_dz}
\end{eqnarray}
where we have defined $P_{i\ell}$ as follows:
\begin{equation}
P_{i\ell}=\frac{\text{exp}\left(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_\ell/\tau\right)}{\sum_{k=1}^{2N}\mathbbm{1}_{i\neq k}\cdot\text{exp}\left(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_\ell/\tau\right)}\ \ \ ,\ \ \ i,\ell\in\{1...2N\}\ ,\ i\neq\ell \nonumber
\end{equation}
$P_{i\ell}$ is the $\ell$'th component of the temperature-scaled softmax distribution of inner products of representations with respect to anchor $i$ and is thus interpretable as a probability. Note that, were we \emph{not} to normalize the projection network output representations, then Eq. \ref{eq:dloss_dz} would effectively be the gradient used for learning (simply let $\boldsymbol{z}_i$ denote a non-normalized vector). It will be insightful to contrast Eq. \ref{eq:dloss_dz} with the form for the projection network gradient (derived below) in which output representations \emph{are} normalized.

The fact that we are using \emph{normalized} projection network output representations introduces an additional term in Eq. \ref{gradient_chain_ruile}, namely $\partial\boldsymbol{z}_i/\partial\boldsymbol{w}_i$, which has the following form:
\begin{eqnarray}
  \frac{\partial\boldsymbol{z}_i}{\partial\boldsymbol{w}_i} & = & \frac{\partial}{\partial\boldsymbol{w}_i}\left(\frac{\boldsymbol{w}_i}{\Vert\boldsymbol{w}_i\Vert}\right) \nonumber \\
  & = & \frac{1}{\Vert\boldsymbol{w}_i\Vert}\cdot\text{I}-\boldsymbol{w}_i\cdot\left(\frac{\partial\left(1/\Vert\boldsymbol{w}_i\Vert\right)}{\partial\boldsymbol{w}_i}\right)^T \nonumber \\
  & = & \frac{1}{\Vert\boldsymbol{w}_i\Vert}\left(\text{I}-\frac{\boldsymbol{w}_i\cdot\boldsymbol{w}_i^T}{\Vert\boldsymbol{w}_i\Vert^2}\right) \nonumber \\
  & = & \frac{1}{\Vert\boldsymbol{w}_i\Vert}\left(\text{I}-\boldsymbol{z}_i\cdot\boldsymbol{z}_i^T\right) \label{dz_dx}
\end{eqnarray}
where I is the identity matrix. Substituting Eqs. \ref{eq:dloss_dz} and \ref{dz_dx} into Eq. \ref{gradient_chain_ruile} gives the following expression for the gradient wrt the \emph{normalized} projection network output representations:
\begin{eqnarray}
  \frac{\partial\mathcal{L}_i^{sup}}{\partial\boldsymbol{w}_i} & = & \frac{-1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau}\cdot\frac{1}{\Vert\boldsymbol{w}_i\Vert}\left(\text{I}-\boldsymbol{z}_i\cdot\boldsymbol{z}_i^T\right)\nonumber\\
  & & \cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  \left(
    (1-P_{ij})\cdot\boldsymbol{z}_j-\sum_{k=1}^{2N}\mathbbm{1}_{k\notin\{i,j\}}\cdot\boldsymbol{z}_k\cdot P_{ik}
  \right) \nonumber \\
  & = & \frac{1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau\cdot\Vert\boldsymbol{w}_i\Vert}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  ((\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j)\cdot\boldsymbol{z}_j-\boldsymbol{z}_j)(1-P_{ij}) \nonumber \\
  & & + \frac{1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau\cdot\Vert\boldsymbol{w}_i\Vert}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  \sum_{k=1}^{2N}\mathbbm{1}_{k\notin\{i,j\}}\cdot(\boldsymbol{z}_k-(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_k)\cdot\boldsymbol{z}_k)\cdot P_{ik} \nonumber \\
  & = & \left.\frac{\partial\mathcal{L}_i^{sup}}{\partial\boldsymbol{w}_i}\right\vert_\text{pos}+\left.\frac{\partial\mathcal{L}_i^{sup}}{\partial\boldsymbol{w}_i}\right\vert_\text{neg} \nonumber
\end{eqnarray}
where:
\begin{eqnarray}
  \left.\frac{\partial\mathcal{L}_i^{sup}}{\partial\boldsymbol{w}_i}\right\vert_\text{pos} & = & \frac{1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau\cdot\Vert\boldsymbol{w}_i\Vert}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  ((\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j)\cdot\boldsymbol{z}_j-\boldsymbol{z}_j)(1-P_{ij}) \nonumber \\
  \left.\frac{\partial\mathcal{L}_i^{sup}}{\partial\boldsymbol{w}_i}\right\vert_\text{neg} & = & \frac{1}{(2N_{\boldsymbol{\tilde{y}}_i}-1)\cdot\tau\cdot\Vert\boldsymbol{w}_i\Vert}\cdot\sum_{j=1}^{2N}\mathbbm{1}_{i\neq j}\cdot\mathbbm{1}_{\boldsymbol{\tilde{y}}_i=\boldsymbol{\tilde{y}}_j}\cdot
  \sum_{k=1}^{2N}\mathbbm{1}_{k\notin\{i,j\}}\cdot(\boldsymbol{z}_k-(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_k)\cdot\boldsymbol{z}_k)\cdot P_{ik} \nonumber
\end{eqnarray}

As discussed in detail in the main paper, for hard positives (i.e., $\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j\approx0$), the $((\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j)\cdot\boldsymbol{z}_j-\boldsymbol{z}_j)(1-P_{ij})$ structure present in $\left.\partial\mathcal{L}_i^{sup}/\partial\boldsymbol{w}_i\right\vert_\text{pos}$ results in large gradients while for easy positives ($\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j\approx1$), it results in small gradients. Analogously, for hard negatives ($\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j\approx0$), the $(\boldsymbol{z}_k-(\boldsymbol{z}_i\bigcdot\boldsymbol{z}_k)\cdot\boldsymbol{z}_k)\cdot P_{ik}$ structure present in $\left.\partial\mathcal{L}_i^{sup}/\partial\boldsymbol{w}_i\right\vert_\text{neg}$ results in large gradients while for easy negatives ($\boldsymbol{z}_i\bigcdot\boldsymbol{z}_j\approx-1$), it results in small gradients. Comparing $\left.\partial\mathcal{L}_i^{sup}/\partial\boldsymbol{w}_i\right\vert_\text{pos}$ and $\left.\partial\mathcal{L}_i^{sup}/\partial\boldsymbol{w}_i\right\vert_\text{neg}$ to that of Eq. \ref{eq:dloss_dz}, one can see that normalizing the projection network output representations served to introduce the general $((\boldsymbol{z}_i\bigcdot\boldsymbol{z}_\ell)\cdot\boldsymbol{z}_{\ell}-\boldsymbol{z}_{\ell})$ structure, which plays a key role in ensuring the gradients are large for hard positives and negatives.

==> impact.tex <==
\section*{Broader Impact}

This work provides a technical advancement in the field of supervised classification, which already has tremendous impact throughout industry. Whether or not they realize it, most people experience the results of this type of classifier many times a day.

As we have shown, supervised contrastive learning can improve both the accuracy and robustness of classifiers, which for most applications should strictly be an improvement. For example, an autonomous car that makes a classification error due to data distribution shift can result in catastrophic results. Thus decreasing this class of error undoubtedly promotes safety. Human driver error is a massive source of fatalities around the world, so improving the safety of autonomous cars furthers the efforts of replacing human drivers. The flip side of that progress is of course the potential for loss of employment in fields like trucking and taxi driving. Similar two-sided coins can be considered for assessing the impact of any application of classification.

An additional potential impact of our work in particular is showing the value of training with large batch sizes. Generally, large batch size training comes at the cost of substantial energy consumption, which unfortunately today requires the burning of fossil fuels, which in turn warms our planet. We are proud to say that the model training that was done in the course of this research was entirely carbon-neutral, where all power consumed was either green to start with, or offset by purchases of green energy. There is unfortunately no way to guarantee that once this research is publicly available that all practitioners of it will choose, or even have the ability to choose, to limit the environmental impact of their model training.

\section*{Acknowledgments and Disclosure of Funding}

Additional revenues related to this work: In the past 36 months, Phillip Isola has had employment at MIT, Google, and OpenAI; honorarium for lecturing at the ACDL summer school in Italy; honorarium for speaking at GIST AI Day in South Korea. P.I.'s lab at MIT has been supported by grants from Facebook, IBM, and the US Air Force; start up funding from iFlyTech via MIT; gifts from Adobe and Google; compute credit donations from Google Cloud.

